Dynamic Graph Message Passing Networks for Visual Recognition

Modelling long-range dependencies is critical for scene understanding tasks in computer vision. Although convolution neural networks (CNNs) have excelled in many vision tasks, they are still limited in capturing long-range structured relationships as they typically consist of layers of local kernels. A fully-connected graph, such as the self-attention operation in Transformers, is beneficial for such modelling, however, its computational overhead is prohibitive. In this paper, we propose a dynamic graph message passing network, that significantly reduces the computational complexity compared to related works modelling a fully-connected graph. This is achieved by adaptively sampling nodes in the graph, conditioned on the input, for message passing. Based on the sampled nodes, we dynamically predict node-dependent filter weights and the affinity matrix for propagating information between them. This formulation allows us to design a self-attention module, and more importantly a new Transformer-based backbone network, that we use for both image classification pretraining, and for addressing various downstream tasks (object detection, instance and semantic segmentation). Using this model, we show significant improvements with respect to strong, state-of-the-art baselines on four different tasks. Our approach also outperforms fully-connected graphs while using substantially fewer floating-point operations and parameters. Code and models will be made publicly available at https://github.com/fudan-zvg/DGMN2

==> figures/DGMN2_sampled_node_visualization.tex <==
\begin{figure*}
	\centering
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis1.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis2.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis3.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis4.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis5.jpg}
	} \\
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis6.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis7.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis8.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis9.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis10.jpg}
	} \\
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis11.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis12.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis13.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis14.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis15.jpg}
	} \\
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis16.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis17.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis18.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis19.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis20.jpg}
	} \\
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis21.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis22.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis23.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis24.jpg}
	}
	\subfloat{
	\includegraphics[width=0.185\linewidth]{./images/DGMN2/Visualization_of_sampled_node/vis25.jpg}
	}
	\caption{
	\small
	Visualization of dynamic sampled graph nodes with our DGMN2 (trained for image classification on ImageNet). The \textcolor{blue}{blue} circle denotes a randomly selected position on observed feature and the \textcolor{orange}{orange} circles denote the corresponding sampled graph nodes. The radii of the \textcolor{orange}{orange} circles indicate the value of the dynamic filters of the sampling graph nodes.
	}
	\label{fig:dgmn2_sampled_node_visualization}
\end{figure*}


==> tables/coco_multiple_dgmn.tex <==
\begin{table}[!t]
\centering
\caption{Quantitative results of inserting proposed module into multiple layers of the ResNet-50.
C3, C4 and C5 denote inserting DGMN after all $3 \times 3$ convolutional layers in \emph{res3}, \emph{res4} and \emph{res5} respectively.
Results are presented for object detection and instance segmentation on COCO 2017 validation set.}
\label{tab:detstage}
\small
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{l|ccc|ccc}
\toprule
Model  & $\mathrm{AP^{box}}$ & $\mathrm{AP^{box}_{50}}$ & $\mathrm{AP^{box}_{75}}$ &$\mathrm{AP^{mask}}$ &$\mathrm{AP^{mask}_{50}}$ &$\mathrm{AP^{mask}_{75}}$  \\
\midrule
Mask R-CNN baseline~\citep{maskrcnn}     &37.8&59.1 &41.4 &34.4  &55.8 &36.6 \\
\midrule
+ GC (C5) ~\citep{cao2019gcnet}    &38.7 &61.1 &41.7 &35.2 &57.4 &37.4 \\ 
+ DGMN (C5)  &\textbf{40.0}&\textbf{62.0} &\textbf{43.5} &\textbf{36.0}  &\textbf{58.5} &\textbf{38.1} \\
\midrule
+ GC (C3, C4, C5) ~\citep{cao2019gcnet}    &39.9 &62.2 &42.9 &36.2 &58.7 &38.3 \\
+ DGMN w/ RWS (C3, C4, C5) &40.7 &62.4 &44.6 &36.8 &59.1 &\textbf{39.5} \\
+ DGMN (C3, C4, C5) &\textbf{41.0}  &\textbf{63.1}  & \textbf{44.8} &\textbf{36.8}  &\textbf{59.6} &39.3 \\

\bottomrule
\end{tabular}
}
\label{tab:c4c5}
\end{table}

==> tables/cs_tables.tex <==
\begin{table}[t]
	\centering
	{\tablestyle{2pt}{1.2}
		\begin{tabular}{ l|x{34}x{34}x{34} }
		&  mIoU (\%)  &   Params &   FLOPs \\
			\shline
			Dilated FCN~\cite{yu2015multi}  & 75.0 &  -- &  --\\
            \hline
             + Deformable~\cite{zhu2018deformable} & 78.2 & +1.31M  &+12.34G \\
             + ASPP~\cite{deeplabv3} &78.9&  +4.42M & +38.45G \\
             + Non-local~\cite{wang2018nonlocal}     &  79.0 & +2.88M & +73.33G\\
            \hline
             + DGMN w/ DA   & 76.5   & +0.57M & +5.32G\\
             + DGMN w/ DA+DW   & 79.1   & +0.73M & +6.88G\\
             + DGMN w/ DA+DW+DS   & \textbf{80.4}   & +3.02M & +28.45G\\
            \multicolumn{4}{c}{~}\\
		\end{tabular}
	}
	\hspace{-2cm}
	\caption{Ablation study on the Cityscapes validation set for semantic segmentation. All models have a ResNet-101 backbone and are evaluated at a single scale.}
	\label{tab:ablation_study_cityscapes}
\end{table}

\begin{table}[t]
	\centering
	\label{tab:city_test}{
		\tablestyle{1pt}{1}
		\begin{tabular}{l |x{42}|x{42}}
			&\scriptsize Backbone &\scriptsize mIoU (\%) \\
			\shline
			\scriptsize PSPNet~\cite{pspnet}   &\scriptsize R101  &\scriptsize 78.4\\
            \scriptsize PSANet~\cite{psanet} &\scriptsize R101  &\scriptsize 80.1   \\
            \scriptsize DenseASPP~\cite{denseaspp} &\scriptsize D161   &\scriptsize 80.6   \\
            \hline
            \scriptsize GloRe~\cite{graph_reason} &\scriptsize R101  &\scriptsize 80.9  \\
            \scriptsize Non-local~\cite{wang2018nonlocal} &\scriptsize R101 &\scriptsize 81.2 \\
            \scriptsize CCNet~\cite{huang2018ccnet} &\scriptsize R101 &\scriptsize 81.4 \\
            \scriptsize DANet~\cite{DAnet} &\scriptsize R101     &\scriptsize 81.5   \\
            \scriptsize DGMN (Ours)  &\scriptsize R101   &\scriptsize \bf 81.8   \\ 
		\end{tabular}}
	\caption{
	Comparison to state-of-the-art for semantic segmentation on Cityscapes.
	All methods are trained with the finely-annotated data from the training and validation sets.
	}
	\label{tab:city}
\end{table}

